Quantum Correlations in Field Theory and Integrable Systems

In this PhD thesis we investigate some properties of one-dimensional quantum systems, focusing on two important aspects of integrable models: Their entanglement properties at equilibrium and their dynamical correlators after a quantum quench. The first part of the thesis will therefore be devoted to the study of the entanglement entropy in one-dimensional integrable systems, with a special focus on the XYZ spin-1/2 chain, which, in addition to being integrable, is also an interacting theory with non perturbative solutions. We derive its bipartite Renyi entropies in the thermodynamic limit and its behaviour in different phases and for different values of the mass-gap is analysed, both analytically and numerically. In particular it is worth mentioning that the numerical analysis of the entropies of the XYZ model presented in this dissertation has never been published in literature. In the second part of the thesis we study the dynamics of correlators after a quantum quench, preparing the system in a squeezed coherent initial state. The emphasis will be on the Transverse Field Ising Chain and the O(3) non-linear sigma model, the latter studied by means of the semi-classical theory, the former by a form-factor approach. Moreover in the last chapter we outline a general result about the dynamics of correlation functions of local observables after a quantum quench. In particular we show that if there are not long-range interactions in the final Hamiltonian, then the dynamics of the model at long times (non equal- time correlations) is described by the same statistical ensemble that describes its statical properties (equal-time correlations). For the Transverse Field Ising Chain this result means that its dynamics is described by a Generalized Gibbs Ensemble.

==> Abstract/abstract.tex <==

% Thesis Abstract -----------------------------------------------------


%\begin{abstractslong}    %uncommenting this line, gives a different abstract heading
\begin{abstract}        %this creates the heading for the abstract page

This is where you write your abstract ...


\end{abstracts}
%\end{abstractlongs}


% ----------------------------------------------------------------------


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 


==> Chapter2/chapter2backup.tex <==
\chapter{Exact entanglement entropy of the XYZ model}
\ifpdf
    \graphicspath{{Chapter2/Chapter2Figs/PNG/}{Chapter2/Chapter2Figs/PDF/}{Chapter2/Chapter2Figs/}}
\else
    \graphicspath{{Chapter2/Chapter2Figs/EPS/}{Chapter2/Chapter2Figs/}}
\fi
In this chapter we will study the Renyi entropy of the one-dimensional XYZ spin-$1/2$ chain in the entirety of its phase diagram. The model has several quantum critical lines corresponding to rotated XXZ chains in their paramagnetic phase, and four tri-critical points where these phases join.
Two of these points are described by a conformal field theory and close to them the entropy scales as the logarithm of its mass gap.
The other two points are not conformal and the entropy has a peculiar singular behavior in their neighbors, characteristic of an {\it essential singularity}. At these non-conformal points the model undergoes a discontinuous transition, with a level crossing in the ground state and a quadratic excitation spectrum.
Moreover we will see how to parametrize the whole phase diagram by using elliptic functions, and in particular how points with the same values of the entropy lying in different phases are connected throught a modular transformation. This approach results to be completely equivalent to the Baxter reparametrization procedure.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Definition of the model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\markboth{\MakeUppercase{\thechapter. Exact entanglement entropy of the XYZ model }}{\thechapter. Exact entanglement entropy of the XYZ model }
We will consider the quantum spin-$\frac{1}{2}$ ferromagnetic XYZ chain, which is described by the following Hamiltonian
\begin{equation}
   H_{XYZ} =
   -{\displaystyle \sum_{n}} \left( J_{x}\sigma_{n}^{x} \sigma_{n+1}^{x}
   + J_{y}\sigma_{n}^{y} \sigma_{n+1}^{y} + J_{z}\sigma_{n}^{z} \sigma_{n+1}^{z} \right) \; ,
   \label{eq:XYZ1}
\end{equation}
where the $\sigma_{n}^{\alpha}$ ($\alpha=x,y,z$) are the Pauli matrices acting on the site $n$, the sum ranges over all sites $n$ of the chain and the constants $J_{x}$, $J_{y}$ and $J_{z}$ take into account
the degree of anisotropy of the model. Without any loss of generality, we can rescale the energy and set $J_{x}=1$.
In the following we will exploit the very well known connection between the XYZ model and the zero-field eight vertex model \cite{Baxter}.
Indeed, as shown by Sutherland \cite{Sutherland}, when the coupling constants of the XYZ model are related to the parameters $\Gamma$ and $\Delta$ of the eight vertex model %
\footnote{On the relation among $\Gamma,\Delta$ and the Boltzmann weights of
XYZ we adopt here the conventions of \cite{Baxter}. %
} at zero external field by the relations
\begin{equation}
   J_{x}:J_{y}:J_{z}=1:\Gamma:\Delta \; ,
   \label{eq:XYZ4bis}
\end{equation}
the row-to-row transfer matrix $T$ of the latter model commutes with the Hamiltonian $H$ of the former.
In the principal regime of the eight vertex model it is customary \cite{Baxter} to parametrize the constants $\Gamma$ and $\Delta$ in terms of elliptic functions
\begin{equation}
   \Gamma = \frac{1+k\;\mbox{sn}^{2}(\ii \lambda)}{1-k\;\mbox{sn}^{2}(\ii \lambda)} \; ,
   \qquad\qquad
   \Delta = -\frac{\mbox{cn}(\ii \lambda)\;\mbox{dn}(\ii \lambda)}{1-k\;\mbox{sn}^{2}(\ii \lambda)} \; ,
   \label{eq:XYZ3bis}
\end{equation}
where $\mbox{sn}(x)$, $\mbox{cn}(x)$ and $\mbox{dn}(x)$ are Jacobian elliptic functions of parameter $k$, while $\lambda$ and $k$ are parameters whose domains are the following
\begin{equation}
   0<k<1\qquad,\qquad 0<\lambda<I(k') \; ,
   \label{eq:XYZ4}
\end{equation}
$I(k')$ being the complete elliptic integral of the first kind of argument $k'=\sqrt{1-k^{2}}$.

We recall that this parametrization is particularly suitable to describe the anti-ferroelectric phase of the eight vertex model, corresponding to $\Delta<-1$. However, using the symmetries of the model and the freedom under the rearrangement of parameters, it can be used in all cases by re-defining the relations that hold between $\Delta$ and $\Gamma$ and the Boltzmann weights (for more details see \cite{Baxter}). Applying these transformations allows us to write the physical parameters of the XYZ model in the whole of the phase diagram in a fairly compact way. In fact, when $\left|J_{y}\right|<1$ and $\left|J_{z}\right|<1$ we have:
\begin{equation}
   \label{st11}
   \begin{cases}
      \Gamma =
      {\displaystyle\frac{ \left| J_z - J_y \right| - \left| J_z + J_y \right| }
      {\left| J_z - J_y \right| + \left| J_z + J_y \right|}} \; , \\
      \Delta =
      {\displaystyle-\frac{2}{\left| J_z - J_y \right| + \left| J_z + J_y \right|}},
   \end{cases}
\end{equation}\\
while for $\left|J_{y}\right|>1$ or $\left|J_{z}\right|>1$, we get:
\begin{equation}
   \label{st12}
   \begin{cases}
      \Gamma =
      {\displaystyle\frac
      {\min\left[2,\left||J_z - J_y\right| - \left|J_z + J_y|\right|\right]}
      {\max\left[2,\left||J_z - J_y\right| - \left|J_z + J_y|\right|\right]}
      \cdot \mbox{sgn} \left[\left|J_z -J_y\right| - \left|J_z + J_y\right|\right]},\\
      \, \\
      \Delta =
      {\displaystyle-\frac{\left|J_z - J_y\right| + \left|J_z + J_y\right|}
      {\max\left[2,\left||J_z - J_y \right| - \left|J_z + J_ y |\right|\right]}},
   \end{cases}
\end{equation}
where $\Gamma$ and $\Delta$ are given by (\ref{eq:XYZ3bis}).
For instance, for $|J_y| \le 1$ and $J_z \le-1$ we recover $J_y = \Gamma$ and $J_z = \Delta$, while for $J_y \ge 1$ and $|J_z| \le 1$ we get $J_y = - \Delta$ and $J_z = -\Gamma$.
In section \ref{sect:newparameters} we show an alternative parametrization of the phase-diagram of the XYZ model, based entirely on the transformation properties of the elliptic functions.

\begin{figure}[t]
   \begin{center}
      \includegraphics[width=8cm]{phaseXYZ}
      \par
   \end{center}
   \caption{Phase Diagram of the XYZ model in the $(J_y, J_z)$ plane. Red lines indicate phase transitions, while the green and blue ones are lines of antiferromagnetic and ferromagnetic order respectively.}
   \label{fig:phasediagram}
\end{figure}


In figure \ref{fig:phasediagram} we draw a cartoon of the phase diagram of the XYZ model in the $(J_y,J_z)$ plane. To understand it better, let us first look at the $J_y=1$ line. Here we have the familiar XXZ model and we recognize the critical (paramagnetic) phase for $|J_z|<1$ and the (anti-)ferromagnetic Ising phases for $J_z>1$ ($J_z<-1$).
The same physics can be observed for $J_y= -1$. There, one can rotate every other spin by 180 degrees around the x-axis to recover a traditional XXZ model. Note, however, that $J_z$ changes sign under this transformation and therefore the ferromagnetic and anti-ferromagnetic Ising phases are respectively for $J_z<-1$ and $J_z>1$.
If we look at the lines $J_z = \pm 1$, we are observing a XYX model, i.e. a rotated XXZ model. Thus the phases are the same as before.
Finally, along the diagonals $J_y = \pm J_z$ we have a XYY model of the form
\be
   H_{XYY} =
   -{\displaystyle \sum_{n}} \left[ \sigma_{n}^{x} \sigma_{n+1}^{x}
   + J_{y} \left( \sigma_{n}^{y} \sigma_{n+1}^{y} + \sigma_{n}^{z} \sigma_{n+1}^{z} \right) \right] \; .
   \label{HXYY}
\ee
Thus the paramagnetic phase is for $|J_y|>1$ and the Ising phases for $|J_y|<1$ with the ferromagnetic one for $J_y = J_z$ and the anti-ferromagnetic one when $J_y = - J_z$.

Thus, in this phase diagram we find four {\it tri-critical points} at $(J_y,J_z) = (\pm 1, \pm 1)$.
As each paramagnetic phase can be described as a sine-Gordon theory with $\beta^{2} = 8 \pi$ at the anti-ferromagnetic isotropic point, flowing to a $\beta^{2} = 0$ theory at the ferromagnetic Heisenberg point, and the critical nature of these tri-critical points is quite different. At $C_{1}=(J_y,J_z) = (1, - 1)$ and $C_{2}=(J_y,J_z) = (- 1, 1)$ we have two conformal points dividing three equivalent sine-Gordon theories with $\beta^{2} = 8 \pi$. At $E_{1}=(J_y,J_z) = (1, 1)$ and $E_{2}=(J_y,J_z) = (- 1, - 1)$, we have two $\beta^{2} = 0$ points which are no longer conformal, since the low energy excitations have a quadratic spectrum there. The former points correspond to an antiferromagnetic Heisenberg chain at the BKT transition, whilst the latter correspond to an Heisenberg ferromagnet at its first order phase transition. 

We will see that the different nature of the tri-critical points will bring dramatic changes in the behavior of the entropy close to them.

Looking at the phase diagram it is evident that it is invariant under reflections with respect to the diagonals $J_y = \pm J_z$. This can be seen at the level of the Hamiltonian, since, for instance, a rotation of the spins by 90 degrees along the x-axis, followed by the exchange $J_y \leftrightarrow J_z$ leaves the Hamiltonian unchanged and the same is valid for a rotation of every other spin by 180 degrees along the x-axis, followed by the reversal of the signs: $J_y \to - J_y$ and $J_z \to - J_z$. Thus we conclude that the thermodynamic quantities of the model (including the entropy) depend only on the parameters $\eta \equiv |J_z + J_y|$ ad $\zeta \equiv |J_z - J_y|$.

Thus, it would be sufficient to describe the model only within one of the four quadrants comprised between the diagonals. However, since interesting points lie on the boundaries of these quadrants, in the following we will concentrate mainly on the $J_y \ge 0$ space, remembering that $J_y <0$ can be recovered by symmetry.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Von Neumann and Renyi entropies}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We are now interested in studying the entanglement properties of the XYZ model in the thermodynamic limit. To this extend, we start with its ground state $\mid0\,\rangle\in\mathcal{H}$ and divide the system in two parts, which we take as the semi-infinite left and right chains, such that $\mathcal{H}=\mathcal{H}_{R}\otimes\mathcal{H}_{L}$ (here we prefer to use the notation $R$ and $L$ instead of $A$ and $B$ for the two subsystems). Then we introduce the density matrix of the whole system $\rho\equiv \mid0\,\rangle\langle\,0\mid$, and trace out one of the two half-chain:
\begin{equation}
   \rho_{R}={\rm Tr}_{\mathcal{H}_{L}}(\rho).
   \label{added}
\end{equation}

According to \cite{Nishino1,Nishino2,Peschel1}, in the thermodynamic limit we can calculate the reduced
density matrix $\rho_{R}$ as product of the four Corner Transfer Matrices $A=C$
and $B=D$ of the eight vertex model at zero field:
\begin{equation}
   \rho_{R}(\bar{\sigma},\bar{\sigma}')
   = (ABCD)_{\bar{\sigma},\bar{\sigma}'}
   = (AB)_{\bar{\sigma},\bar{\sigma}'}^{2} \; ,
   \label{eq:XYZ4a}
\end{equation}
where $\bar{\sigma}$ and $\bar{\sigma}'$ are particular spin configurations of the semi-infinite chain.\\
Generally speaking, the above quantity does not satisfy the constraint ${\rm Tr}\rho_{R}=1$, so we must consider a normalized version $\rho_{R}'$.
Notice taking the trace of the reduced density matrix over the remaining half-line we get the normalization of $\rho_{R}$, which corresponds to the partition function of the eight vertex model:
\be
   \mathcal{Z} \equiv {\rm Tr}\rho_{R}.
   \label{Zdef}
\ee

For the zero field eight vertex model with fixed boundary conditions, Baxter constructed an explicit form of the Corner Transfer Matrices (CTM's) in the thermodynamic limit \cite{Baxter,Baxter1,Baxter2}. In \cite{Evangelisti} it was shown that, using relation (\ref{eq:XYZ4a}), the reduced density operator can be written as
\begin{equation}
   \rho_{R}=\left(\begin{array}{cc}
        1 & 0\\
        0 & x^{2}\end{array}\right)
   \otimes\left(\begin{array}{cc}
        1 & 0\\
        0 & x^{4}\end{array}\right)
   \otimes\left(\begin{array}{cc}
        1 & 0\\
        0 & x^{6}\end{array}\right)
   \otimes \ldots \; ,
   \label{eq:XYZ6}
\end{equation}
where $x \equiv \exp[-\pi\lambda/2I(k)]$.
We notice that $\rho_{R}$ is a function of $\lambda$ and $k$ only through $x$.
Furthermore, (\ref{eq:XYZ6}) can be rewritten as
\begin{equation}
   \rho_{R}=(AB)^{2}=\eu^{-\epsilon\hat{O}} \; .
   \label{eq:XYZ7}
\end{equation}
$\hat{O}$ is an operator with integer eigenvalues ( which was defined before equation (\ref{chap1_eq24})) and also:
\begin{equation}
   \epsilon \equiv \pi \: {\lambda \over 2I(k)} \; .
   \label{eq:eps}
\end{equation}
The Von Neumann entropy ${\cal S}$ can be calculated easily according to (\ref{chap1_eq24}):
\begin{equation}
   {\cal S}
   = -\mbox{Tr}\rho_{R}'\ln\rho_{R}'
   = -\epsilon{\displaystyle \frac{\partial\ln\mathcal{Z}}{\partial\epsilon}}+\ln\mathcal{Z} \; ,
   \label{eq:XYZ8}
\end{equation}
where the partition function can be written as
\begin{equation}
   \mathcal{Z} = {\displaystyle \prod_{j=1}^{\infty}}(1+x^{2j})
   = {\displaystyle \prod_{j=1}^{\infty}}(1+\eu^{-\pi j \lambda/I(k)}) \; .
   \label{eq:XYZ9}
\end{equation}
Thus we obtain an exact analytic expression for the entanglement entropy of the XYZ model as
\begin{equation}
   {\cal S} = 2\epsilon{\displaystyle \sum_{j=1}^{\infty}}{\displaystyle \frac{j}{(1+\eu^{2j\epsilon})}}
   + {\displaystyle \sum_{j=1}^{\infty}}\ln(1+\eu^{-2j\epsilon}) \; ,
   \label{eq:XYZ10}
\end{equation}
which is valid for generic values of $\lambda$ and $k$. 
Another quantity of interest to quantify the entanglement is the Renyi entropy
\begin{equation}
   {\cal S}_{\alpha} \equiv {\displaystyle\frac{1}{1-\alpha}}\ln\mbox{Tr}[\rho_{R}^{\prime \alpha}] \; ,
   \label{eq:renyi1}
\end{equation}
where $\alpha$ is a parameter. 

The Renyi entropy can be seen as a generalized series expansion for the von Neumann entropy and it is directly related to the spectrum of the reduced density matrix, see, for instance, \cite{franchini2010}. As we have already seen, in the limit $\alpha \to 1$ it reduces to the von Neumann entropy.

Using the factorized expression (\ref{eq:XYZ6}) for $\rho$, we can be easily write
\begin{equation}
   \rho_{R}^\alpha=\left(\begin{array}{cc}
        1 & 0\\
        0 & x^{2\alpha}\end{array}\right)
   \otimes\left(\begin{array}{cc}
        1 & 0\\
        0 & x^{4\alpha}\end{array}\right)
   \otimes\left(\begin{array}{cc}
        1 & 0\\
        0 & x^{6\alpha}\end{array}\right)
   \otimes \ldots \; .
   \label{eq:renyi2}
\end{equation}
With this result and noting that
\begin{equation}
   \label{eq:renyi3}
   \mbox{Tr}\rho_{R}^{\prime \alpha} =
   \mbox{Tr}\left ({\displaystyle\frac{\rho_{R}}{\mathcal{Z}}}\right)^{\alpha} =   {\displaystyle\frac{\mbox{Tr}\rho_{R}^{\alpha}}{\mathcal{Z}^{\alpha}} } =  {\displaystyle\frac{\prod_{j=1}^{\infty}\left(1+\eu^{-2j\alpha\epsilon} \right)}{\mathcal{Z}^{\alpha}} } \; ,
\end{equation}
it is now trivial to compute the Renyi entropy of the XYZ model:
\begin{eqnarray}
   {\cal S}_{\alpha}  & = &
   {\displaystyle\frac{1}{1-\alpha}} \left [ \ln {\displaystyle\frac{1}{\mathcal{Z}^{\alpha}}} + \sum_{j=1}^{\infty}\ln \left ( 1+\eu^{-2j\alpha\epsilon}  \right) \right]
   \nonumber \\
%\, & = & {\displaystyle\frac{\alpha}{\alpha-1}}\ln\mathcal{Z} + %{\displaystyle\frac{1}{1-\alpha}}\sum_{j=1}^{\infty}\ln\left ( 1+e^{-j\alpha\epsilon}  \right) \\
   & = & {\displaystyle\frac{\alpha}{\alpha-1}} \sum_{j=1}^{\infty}\ln\left ( 1+\eu^{-2j\epsilon} \right)
   + {\displaystyle\frac{1}{1-\alpha}}\sum_{j=1}^{\infty}\ln\left ( 1+\eu^{-2j\alpha\epsilon} \right) \; .
   \label{eq:renyi4}
\end{eqnarray}
Moreover, by introducting the generalized partition function:
\be
   \mathcal{Z}_{\alpha} 
   = {\displaystyle \prod_{j=1}^{\infty}}(1+\eu^{-2j\alpha\epsilon})\;.
   \label{eq:XYZ10bis}
\ee
we can re-write the Von Neumann entropy as:
\be
   {\cal S}=\left.\left(1-\frac{\partial}{\partial\alpha}\right) \ln\mathcal{Z}_{\alpha}\right|_{\alpha = 1}
   \label{eq:XYZ10tris}
\ee
and the Renyi entropy as:
\be
   {\cal S}_{\alpha}=\lim_{\beta\to 1}{\displaystyle\frac{\beta\ln\mathcal{Z}_{\alpha}-\alpha\ln\mathcal{Z}_{\beta}}{\beta-\alpha}}\;.
   \label{eq:XYZ10quatris}
\ee
These two last expressions are completely equivalent to (\ref{eq:XYZ10}) and (\ref{eq:renyi4}) respectively.
When $\epsilon\ll1$, i.e. in the scaling limit analogous to the one of \cite{Weston}, formula (\ref{eq:XYZ10})
can be approximated by its Euler-Maclaurin asymptotic expansion which was introduced in (\ref{chap1_eq30}), yielding
\begin{eqnarray}
{\cal S} & = & {\displaystyle \int_{0}^{\infty}}\;{\rm d}x\;\left({\displaystyle \frac{x\epsilon}{1+e^{x\epsilon}}}+\ln(1+e^{-x\epsilon})\right)-{\displaystyle \frac{\ln2}{2}}+O(\epsilon)\nonumber \\
\, & = & {\displaystyle \frac{\pi^{2}}{6}}{\displaystyle \frac{1}{\epsilon}}-{\displaystyle \frac{\ln2}{2}}+O(\epsilon)
\label{eq:XYZ11}
\end{eqnarray}
This will be used in the next subsection where we will check our analytic results against some special known cases, namely the XXZ and
the XY chain.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The XXZ and XY spin-$1/2$ chain limits}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us first consider the case $k=0$ (i.e. $\Gamma=1$) and the limit
$\lambda\to 0^{+}$, which corresponds to the spin $1/2$ XXZ. In this
limit the eight vertex model reduces to the six vertex model. Let
us note that formula (\ref{eq:XYZ11}) coincides exactly with the
one proposed by Weston \cite{Weston} which was obtained in the study
of more general spin $\kappa/2$. In this limit the approximation
$\epsilon\ll1$ is still valid and we can use the result of equation
(\ref{eq:XYZ11}). From relation (\ref{eq:XYZ3bis}), it follows that
\begin{equation}
\lambda={\displaystyle\sqrt{2}}\sqrt{-\Delta-1}+O\left((-1-\Delta)^{3/2}\right)\label{eq:XYZ12}
\end{equation}
 Thus equation (\ref{eq:XYZ11}) gives\begin{equation}
{\cal S}=\frac{\pi^{2}}{12\sqrt{2}}\,\frac{1}{\sqrt{-\Delta-1}}-\frac{\ln(2)}{2}+O\left((-1-\Delta)^{1/2}\right)\label{eq:XYZ13}\end{equation}
 which can be written in a simpler form if we recall that, when $\epsilon\to0$
(i.e. $\Delta\rightarrow-1^{-}$), the correlation length is given
by \cite{Baxter} 
\begin{equation}
\ln\frac{\xi}{a}={\displaystyle {\frac{\pi^{2}}{2\epsilon}}-2\ln(2)+O(e^{-\pi^{2}/\epsilon})}
\end{equation}
 where $a$ is the lattice spacing. Recalling that \begin{equation}
\epsilon={\displaystyle \sqrt{2}}\sqrt{-\Delta-1}+O\left((-1-\Delta)^{3/2}\right)\end{equation}
 the expression for the entanglement entropy becomes \begin{equation}
{\cal S}=\frac{1}{6}\ln\frac{\xi}{a}+U+O\left((-1-\Delta)^{1/2}\right)\end{equation}
 where $U=-\ln(2)/6$. This last expression confirms the general theory
of equation (\ref{eq:intro1}) with $c=1$, which is exactly what
one should expect, the XXZ model along its critical line being a free
massless bosonic field theory with $c=1$.

As a second check, we consider the case $\Gamma=0$, which corresponds
to the XY chain. It is convenient now to describe the corresponding
eight vertex model by using Ising-like variables which are located
on the dual lattice \cite{Baxter}, thus obtaining an anisotropic
Ising lattice, rotated by $\pi/4$ with respect to the original one,
with interactions round the face with coupling constants $J,J'$,
as shown in figure \ref{fig:ising}. %
\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{doppioising} 
\par\end{center}
\caption{Decoupled anisotropic Ising lattices. Horizontal and vertical lines
belong to the original eight vertex model lattice, diagonal lines
belong to the dual Ising lattice.}
\label{fig:ising} 
\end{figure}


In our case the Ising lattice decouples into two single sublattices
with interactions among nearest neighbors. Now \begin{equation}
\Delta=\sinh(2\beta J)\sinh(2\beta J')\equiv k_{I}^{-1}\label{eq:XYZ17}\end{equation}
 so that, using the elliptic parametrization, one has\begin{equation}
\lambda=\frac{1}{2}I(k')\label{eq:XYZ18}\end{equation}
 Thus $\epsilon$ of equation (\ref{eq:eps}) becomes \begin{equation}
\epsilon=\frac{\pi I(k_{I}')}{2I(k_{I})}\label{eq:XYZ19}\end{equation}
 Let us approach the critical line of the anisotropic Ising model
from the ferromagnetic phase, i.e. let us assume that $k_{I}\to1^{-}$.
In this case it is straightforward to write \begin{equation}
\epsilon=-{\displaystyle \frac{\pi^{2}}{2\ln(1-k_{I})}}+O\left(\ln^{-2}(1-k_{I})\right)\label{eq:XYZ20}\end{equation}
 so that the entanglement entropy becomes\begin{equation}
{\cal S}=-\frac{1}{6}\ln(1-k_{I})+O\left(\ln^{-1}(1-k_{I})\right)\label{eq:XYZ21}\end{equation}
 Since $\xi^{-1}=(1-k_{I})+O\left((1-k_{I})^{2}\right)$, we can easily
conclude that\begin{equation}
{\cal S}=\frac{1}{6}\ln\frac{\xi}{a}+O\left(\ln^{-1}(1-k_{I})\right)\label{eq:XYZ22}\end{equation}
 where again the leading term confirms the general result (\ref{eq:intro1}),
with $c=1$. This result is in agreement with what found in previous
works \cite{Vidal,Cardy,Peschel3,Korepin, Korepin2} by means of different approaches.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The sine-Gordon limit}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In \cite{Luther,McCoy} it has been proposed that a particular scaling
limit of the XYZ model yields the sine-Gordon theory. In this section
we will use this connection to compute the exact entanglement entropy between
two semi-infinite intervals of a 1+1 dimensional sine-Gordon model.
In his article, Luther \cite{Luther} showed that in the scaling
limit, where $a\to0$ while keeping the mass gap constant, the parameters
of the XYZ model and those of the sine-Gordon theory are connected
by the following relation (keeping $J_{x}=1$ from the beginning)\begin{equation}
M=8\pi\,\left({\displaystyle \frac{\sin\mu}{\mu}}\right)\,\left({\displaystyle \frac{l_{r}}{4}}\right)^{\pi/\mu}\label{eq:SG1}\end{equation}
 where the parameter $\mu$ is defined as\begin{equation}
\mu\equiv\pi\left(1-{\displaystyle \frac{\beta^{2}}{8\pi}}\right)=\arccos\left({\displaystyle -J_{z}}\right)\label{eq:SG2}\end{equation}
 Here $M$ is the sine-Gordon solitonic mass, and $l_{r}=l\, a^{-\mu/\pi}$,
with\begin{equation}
l^{2}={\displaystyle \frac{1-J_{y}^{2}}{1-J_{z}^{2}}}\label{eq:SG3}\end{equation}
 These relations tell us how the coupling constant $J_{z}$ is connected
to the parameter $\beta$ of sine-Gordon, and how $J_{y}$ scales
when we take the scaling limit $a\to0$. It is clear from equation
(\ref{eq:SG3}) that in this limit $J_{y}\to1^{-}$. In the following
we work in the repulsive regime $4\pi<\beta^{2}<8\pi$ (which corresponds
to $0<\mu<\pi/2$ and $-1<J_{z}<0$). In this regime the mass gap
of the theory is the soliton mass $M$. Taking this limit we use the
following parametrization of the XYZ coupling constants\begin{equation}
\Gamma={\displaystyle \frac{J_{z}}{J_{y}}}\qquad,\qquad\Delta={\displaystyle \frac{1}{J_{y}}}\label{eq:SG4}\end{equation}
 which amounts to a reparametrization of the Boltzmann weights of
XYZ suitable for the $|\Delta|\leq1$ disordered regime where we are
working now (see chapter 10 of \cite{Baxter} for details). As a consequence
of such reparametrization a minus sign appears in front of both equations
(\ref{eq:XYZ3bis}). Taking the sine-Gordon limit, $\lambda$ and
$k$ parametrizing $\Gamma$ and $\Delta$ must now satisfy the following
constraint\begin{equation}
\mbox{sn}^{2}(i\lambda)=-{\displaystyle \frac{\frac{J_{z}}{J_{y}}+1}{k-k\frac{J_{z}}{J_{y}}}}\label{eq:SG5}\end{equation}
 Considering the parametrization of $\Delta$ and using the properties
of the Jacobian elliptic functions we can write\begin{equation}
\Delta^{2}=\frac{\mbox{cn}^{2}(i\lambda)\mbox{dn}^{2}(i\lambda)}{(1-k\;\mbox{sn}^{2}(i\lambda))^{2}}={\displaystyle \frac{\left(k(1-\frac{J_{z}}{J_{y}})+\frac{J_{z}}{J_{y}}+1\right ) \left(k(1+\frac{J_{z}}{J_{y}})-\frac{J_{z}}{J_{y}}+1\right)}{4k}}\label{eq:SG6}\end{equation}
 Expanding around $k\to1^{-}$ and collecting $\Delta^{2}=1/J_{y}^{2}$
from both sides of the equation we find\begin{equation}
\Delta^{2}=1+\frac{1}{4}(1-J_{z}^{2})(k-1)^{2}+O(k-1)^{3}\label{eq:SG7}\end{equation}
 Using equation (\ref{eq:SG1}) we obtain\begin{equation}
l^{2}=l_{r}^{2}a^{2\mu/\pi}=4^{2-3\mu/\pi}\left({\displaystyle \frac{M\mu a}{\pi\sin\mu}}\right)^{2\mu/\pi}\label{eq:SG8}\end{equation}
 where $\mu$ is completely fixed by choosing a particular value of
$J_{z}$. Now using the definition (\ref{eq:SG3}) and (\ref{eq:SG4})
we find\begin{equation}
\Delta^{2}=1+(1-J_{z}^{2})4^{2-3\mu/\pi}\left({\displaystyle \frac{M\mu a}{\pi\sin\mu}}\right)^{2\mu/\pi}+O(a^{4\mu/\pi})\label{eq:SG9}\end{equation}
 which is valid when $a\to0$. Comparing equation (\ref{eq:SG7})
with (\ref{eq:SG9}) we can identify in which way $k$ scales to $1^{-}$\begin{equation}
k=1-2^{3(1-\mu/\pi)}\left({\displaystyle \frac{M\mu a}{\pi\sin\mu}}\right)^{\mu/\pi}+O(a^{2\mu/\pi})\label{eq:SG10}\end{equation}
 Remembering the constraint (\ref{eq:SG5}) and using the previous
expression for $k$ we have\begin{equation}
\mbox{sn}^{2}(i\lambda)={\displaystyle \frac{-J_{z}-1}{1-J_{z}}+O(a^{\mu/\pi})}\label{eq:SG11}\end{equation}
 When $k\to1$ the elliptic function sn reduces to an hyperbolic tangent,
thus we obtain\begin{equation}
\tan^{2}\lambda={\displaystyle \frac{1+J_{z}}{1-J_{z}}+O(a^{\mu/\pi})\quad\longrightarrow\quad\lambda=\arctan\sqrt{{\displaystyle \frac{1+J_{z}}{1-J_{z}}}}+O(a^{\mu/\pi})}\label{eq:SG12}\end{equation}
 Now we can evaluate the expression (\ref{eq:XYZ10}) in this limit.
Using the following asymptotic behaviour of the elliptic integral
$I(x)$\begin{equation}
I(x)\approx-\frac{1}{2}\ln(1-x)+\frac{3}{2}\ln2+O(1-x),\qquad x\approx1^{-}\label{eq:SG13}\end{equation}
 along with the approximation (\ref{eq:XYZ11}), we can write the
exact entanglement entropy of a bipartite XYZ model in the sine-Gordon
limit\begin{equation}
{\cal S}_{sG}=-{\displaystyle \frac{\pi}{12}\frac{\ln(1-k)-3\ln2}{\arctan\sqrt{{\displaystyle \frac{1+J_{z}}{1-J_{z}}}}}-{\displaystyle \frac{\ln2}{2}}+O(1/\ln(a))}\label{eq:SG14}\end{equation}
 The leading correction to this expression comes from the $O(\epsilon)$
term of equation (\ref{eq:XYZ11}). The constant $J_{z}$ is connected
to $\beta$ by\begin{equation}
J_{z}=-\cos\pi\left(1-\frac{\beta^{2}}{8\pi}\right)\label{eq:SG15}\end{equation}
 thus using this property and the scaling expression (\ref{eq:SG11})
we can write down the entanglement entropy as\begin{equation}
{\cal S}_{sG}={\displaystyle \frac{1}{6}\ln\left(\frac{1}{Ma}\right)+\frac{1}{6}\ln\left(\frac{\sin\left[\pi\left(1-\frac{\beta^{2}}{8\pi}\right)\right]}{\left(1-\frac{\beta^{2}}{8\pi}\right)}\right)+O(1/\ln(a))}\label{eq:SG16}\end{equation}
 This result confirms the general theory due to \cite{Cardy,Doyon},
in the limit where the system is bipartite in two infinite intervals,
with the central charge equal to 1, as it should, because the sine-Gordon
model can be considered a perturbation of a $c=1$ conformal field
theory (described by a free massless boson compactified on a circle
of radius $\sqrt{\pi}/\beta$) by a relevant operator of (left) conformal
dimension $\beta^{2}/8\pi$. We can write \begin{equation}
{\cal S}_{sG}\approx{\displaystyle \frac{1}{6}\ln\left(\frac{1}{Ma}\right)+U(\beta)\qquad a\to0}\label{eq:SG17}\end{equation}
 where the constant term $U(\beta)$ takes the value \begin{equation}
U(\beta)={\displaystyle \frac{1}{6}\ln\left(\frac{\sin\left[\pi\left(1-\frac{\beta^{2}}{8\pi}\right)\right]}{\left(1-\frac{\beta^{2}}{8\pi}\right)}\right)}\label{eq:SG18}\end{equation}


At $\beta^{2}=4\pi$, when the sine-Gordon model becomes the free
Dirac fermion theory, it assumes the value $U(\sqrt{4\pi})=\frac{1}{6}\log2=0.11552453...$,
while at $\beta^{2}=8\pi$, where the theory becomes a relevant perturbation
of the WZW conformal model of level 1 by its operator of left dimension
$\frac{1}{4}$, it becomes $U(\sqrt{8\pi})=\frac{1}{6}\log\pi=0.19078814...$.\\
 We notice that formula (\ref{eq:SG16}) yields the exact value of
the {\it overall} constant $U(\beta)$, since it has been derived from equation
(\ref{eq:XYZ11}) which is exact up to terms $O(\epsilon)$. As
mentioned in the introduction and as observed by many authors
\cite{Bombelli,Callan,Schumacher,Nishino2}, $U$ should contain a
contribution from the Affleck Ludwig boundary term as well as a
model-dependent constant that will be discussed in the next chapter.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Renyi entropy in terms of theta functions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Expression (\ref{eq:renyi4}) for the entropy is exact in the thermodynamic limit and it is quite convenient for numerical evaluations. However, to better understand the behavior of the entropy we can use a more explicitly analytical expression. This is done by recognizing that (\ref{eq:renyi4}) is essentially a sum of two q-series in the parameter $q= \eu^{-\epsilon}$. These series can be conveniently expressed in terms of Jacobi theta functions, which can be defined by the products
\bea
   \theta_1 (z,q) & = & 2 q^{1/4} \sin z \prod_{j=1}^\infty
   \left( 1 - q^{2j} \right) \left[ 1 - 2 q^{2j} \cos (2z) + q^{4j} \right] \; ,
   \label{theta1def} \\
   \theta_2 (z,q) & = & 2 q^{1/2} \cos z \prod_{j=1}^\infty
   \left( 1 - q^{2j} \right) \left[ 1 + 2 q^{2j} \cos (2z) + q^{4j} \right] \; ,
   \label{theta2def} \\
   \theta_3 (z,q) & = & \prod_{j=1}^\infty
   \left( 1 - q^{2j} \right) \left[ 1 + 2 q^{2j-1} \cos (2z) + q^{4j-2} \right] \; ,
   \label{theta3def} \\
   \theta_4 (z,q) & = & \prod_{j=1}^\infty
   \left( 1 - q^{2j} \right) \left[ 1 - 2 q^{2j-1} \cos (2z) + q^{4j-2} \right] \; .
   \label{theta4def}
\eea

It is then easy to see that we have the identity
\be
   \prod_{j=1}^\infty \left( 1 + q^{2j} \right) =
   \left( { \theta_2^2 (0,q) \over 4 q^{1/2} \theta_3 (0,q) \theta_4 (0,q) } \right)^{1/6} \; .
\ee
With this help, we can write (\ref{eq:renyi4}) as
\bea
   {\cal S}_{\alpha} & = & {\displaystyle\frac{\alpha}{\alpha-1}}
   \ln \prod_{j=1}^{\infty} \left ( 1 + \eu^{-2j\epsilon}  \right)
   + {\displaystyle\frac{1}{1-\alpha}}
   \ln \prod_{j=1}^{\infty} \left ( 1 + \eu^{-2j\alpha\epsilon}  \right)
   \nonumber  \\
   & = & {\alpha \over 6(\alpha -1)}
   \ln{\theta_2^2 (0,q) \over \theta_3 (0,q) \theta_4 (0,q) }
   \nonumber \\
   & + & {1 \over 6(1 - \alpha)}
   \ln{\theta_2^2 (0,q^{\alpha}) \over \theta_3 (0,q^{\alpha}) \theta_4 (0,q^{\alpha}) } - {1 \over 3} \ln 2\; .
   \label{eq:modular2}
\eea
and the Von Neumann entropy as
\bea
   {\cal S} & = & {\displaystyle\frac{1}{6}}
   \ln {\theta_2^2 (0,q) \over \theta_3 (0,q) \theta_4 (0,q) }
   - {\displaystyle\frac{1}{6}} {\de \over \de \alpha} \left. \ln
   {\theta_2^2 (0,q^{\alpha}) \over \theta_3 (0,q^{\alpha}) \theta_4 (0,q^{\alpha}) } \right|_{\alpha =1}
   -\frac{\ln(2)}{3}
   \nonumber \\
   & = & \frac{1}{6} \ln {\theta_2^2 (0,q) \over
   4 \theta_3 (0,q) \theta_4 (0,q) }-\frac{\ln(q)}{2}\left(2\theta_{3}^{4}(0,q)-\theta_{2}^{4}(0,q)\right)
   \label{vonNeumannTheta}
\eea

These expressions for the entropies are completely equivalent to the series we started from and might even appear more complicated.
However, the advantage of expressing them in terms of elliptic function will become apparent in the next sections, where this formulation will allow us to easily study their behavior.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analytical continuation in the upper \\ half-plane of the phase diagram}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sect:newparameters}

In this section we will show that, using some simple transformations for the elliptic functions, we can provide some more compact parametrizations for the parameters of the XYZ model. In particular we will show how to cover the entire plane $(J_{y},J_{z})$ by means of a single parametrization formula, without using the Baxter rearrangement procedure. In addition we will discover that to each analytical continuation there corresponds a modular transformation of a parameter $\tau$. Nonetheless there exists a family of modular transformations that bridge points with the same value of the Renyi entropy that belong to different contour lines of $S_{\alpha}$.\\
In order to show these properties explicitly, it is very useful to introduce a new couple of parameters $(z,l)$ instead of the old ones $(\lambda,k)$, by means of a Landen transformation.  
Using the table of transformation 8.152 of \cite{gradshteyn} we have
\bea
   \Gamma & = & {1 + k \; \sn^2 (\ii \lambda ; k) \over 1 - k \; \sn^2 (\ii \lambda ; k) }
   = {1 \over \dn ( \ii z ; l ) } \; , \\
   \Delta & = & - { \cn (\ii \lambda ; k) \; \dn (\ii \lambda ; k) \over
   1 - k \; \sn^2 (\ii \lambda ; k) }
   = - { \cn (\ii z ; l) \over \dn (\ii z ; l) } \; ,
\eea
where we defined the new parameters
\be
   l \equiv {2 \sqrt{k} \over 1 + k} \; , \qquad \qquad
   z \equiv (1+k) \lambda \; .
   \label{landen}
\ee
In order to describe the principal regime only, it is sufficient to consider the following ranges of the parameters $(z, l)$:
\be
   0 < z < 2I(l')  \qquad \qquad
   0 < l < 1 \; .
\ee
The previous transformation is known as a Landen transformation and we further have the following identities
\be
\label{eps1}
   l' = \sqrt{1 - l^2} = { 1 - k \over 1 +k} \; , \qquad
   I (l) = (1 +k) I (k) \; , \qquad
   I (l') = {1 + k \over 2} I (k') \; .
\ee
Hence we see that
\be
\label{eps2}
   \epsilon = \pi {\lambda \over 2I (k)} = \pi {z \over 2I(l)} ={\pi \over 2\ii}{\tilde{z}\tau}
\ee
where
\be
\label{eps3}
   \tilde{z} \equiv {z \over I (l')}, \qquad \qquad \tau\equiv \ii{I(l') \over I(l)}
\ee
where $0<\tilde{z}<2$ and $\tau \in \mathbb{C}$.
In terms of $\Gamma$ and $\Delta$ of formulae (\ref{st11}) and (\ref{st12}) $(z,l)$ are given by (see \cite{Baxter}, chapter 10):
\begin{equation}
\label{ste8bis}
    \begin{cases}
     l = \displaystyle{\sqrt{ {1-\Gamma^{2} \over \Delta^{2}-\Gamma^{2} } } }\\
     {\rm dn}(\ii z;l) = \displaystyle{1 \over \Gamma} .
    \end{cases}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% QUESTO ERA IL VECCHIO MODO DI CALCOLARE EPSILON, QUELLO NUOVO E MODULARE L'HO MESSO ALLA FINE DELLA SEZIONE MODULARE QUANDO DISCUTO LE PROPRIETA' DI GRUPPO
%In order to compute the Renyi entropy $S_{\alpha}$ in an arbitrary point of the phase diagram, firstly we need to use formulae (\ref{st11}) and (\ref{st12}) to %determine $(\Gamma,\Delta)$, secondly we put these values into equation (\ref{ste8bis}) to obtain $(z,l)$, and finally we extract the value of $\epsilon$ from %(\ref{eps2}). With $\epsilon$ it is straightforward to compute $S_{\alpha}$ by using formula (\ref{eq:modular2}). 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The idea of the analytical continuation is to enlarge the domains of $(\tilde{z}, l)$ in a way that allows us to cover the whole space of parameters $(J_{y},J_{z})$. \\
Let us now look at the part of the phase diagram (${\rm I}_a$ in fig. (\ref{fig:phasediagram})) with $|J_z| \le 1$ and $J_y \ge 1$. This region is completely equivalent to the principal regime, as we defined it before. By using the Baxter rearrangement procedure (\ref{st12}) we have:
\be
\begin{cases}
   J_y (\tilde{z},l) = - \Delta = {\displaystyle{\cn ( \ii \tilde{z} I'(l) ; \,l) \over \dn ( \ii \tilde{z} I'(l) ; \,l ) }} \; \\
   J_z (\tilde{z},{l}) = -\Gamma = -{\displaystyle{1 \over \dn ( \ii \tilde{z} I'(l) ; \,l ) }} \; .
   \label{Iaparameter}
\end{cases}
\ee
Now we want to find a strategy to reach every region in figure (\ref{fig:phasediagram}) with an analytic continuation of formula (\ref{Iaparameter}). We begin by illustrating how to cover the quadrant ${\rm I}$. It is convenient to re-express formula (\ref{Iaparameter}) in terms of Jacobi theta functions. In order to do this, let us introduce the new variable $u = {\pi\tilde{z}\over 2}$. We can express the elliptic functions in terms of theta functions in the following way:
\be
\begin{cases}
  {\rm cn}(\ii\tilde{z}I'|\tau)={\displaystyle\frac{\theta_{4}(0|\tau)}{\theta_{2}(0|\tau)}}{\displaystyle\frac{\theta_{2}(\ii\frac{\pi}{2}\tilde{z}\frac{I'}{I}|\tau)}{\theta_{4}(\ii\frac{\pi}{2}\tilde{z}\frac{I'}{I}|\tau)}}={\displaystyle\frac{\theta_{4}(0|\tau)}{\theta_{2}(0|\tau)}}{\displaystyle\frac{\theta_{2}(u\tau|\tau)}{\theta_{4}(u\tau|\tau)}}\\
  {\rm dn}(\ii\tilde{z}I'|\tau)={\displaystyle\frac{\theta_{4}(0|\tau)}{\theta_{3}(0|\tau)}}{\displaystyle\frac{\theta_{3}(\ii\frac{\pi}{2}\tilde{z}\frac{I'}{I}|\tau)}{\theta_{4}(\ii\frac{\pi}{2}\tilde{z}\frac{I'}{I}|\tau)}}={\displaystyle\frac{\theta_{4}(0|\tau)}{\theta_{3}(0|\tau)}}{\displaystyle\frac{\theta_{3}(u\tau|\tau)}{\theta_{4}(u\tau|\tau)}}
   \label{theta1}
\end{cases}
\ee
Region ${\rm I}_{a}$ is then parametrized by:
\be
\begin{cases}
J_{y}= {\displaystyle\frac{\theta_{3}(w(\tau)|\tau)}{\theta_{2}(w(\tau)|\tau)}}{\displaystyle\frac{\theta_{2}(u\tau|\tau)}{\theta_{3}(u\tau|\tau)}}\\ 
J_{z}= -{\displaystyle\frac{\theta_{3}(w(\tau)|\tau)}{\theta_{4}(w(\tau)|\tau)}}{\displaystyle\frac{\theta_{4}(u\tau|\tau)}{\theta_{3}(u\tau|\tau)}}
\label{theta2}
\end{cases}
\ee
where $0<u<\pi/2$ and $w(\tau) \in (0,\,\pi\tau)$ in the left-side and right-side of region ${\rm I}_{a}$ respectively. In practice we are using two parametrization for the left and right subsystems of the principal regime. At this point this could seem a useless complication, but we will soon see that parametrizing the fundamental domain this way allows us to cover the whole phase diagram by means of very simple transformations of the parameters $(u,\tau)$. 
In general we can identify a specific point of a particular region of the {\em upper half-plane} $J_{y}\geq 0$ of the phase diagram by specify the pair of parameters $(u,\tau)$\footnote{We will discuss how to cover the {\em lower half-plane} $J_{y}\leq 0$ phase diagram in the next section.}.
Now by using the properties of the Jacobi theta functions under the action of the modular group it is possible to cover all other regions in the upper half-plane (see the appendix for a brief reminder of these properties). Let us start by region ${\rm I}_b$:
\be
\begin{cases}
J_{y}= {\displaystyle\frac{\theta_{3}(0|\tau+1)}{\theta_{2}(0|\tau+1)}}{\displaystyle\frac{\theta_{2}(u\tau|\tau+1)}{\theta_{3}(u\tau|\tau+1)}}={\displaystyle\frac{\theta_{4}(0|\tau)}{\theta_{2}(0|\tau)}}{\displaystyle\frac{\theta_{2}(u\tau|\tau)}{\theta_{4}(u\tau|\tau)}}\\ 
J_{z}= -{\displaystyle\frac{\theta_{3}(0|\tau+1)}{\theta_{4}(0|\tau+1)}}{\displaystyle\frac{\theta_{4}(u\tau|\tau+1)}{\theta_{3}(u\tau|\tau+1)}}=-{\displaystyle\frac{\theta_{4}(0|\tau)}{\theta_{3}(0|\tau)}}{\displaystyle\frac{\theta_{3}(u\tau|\tau)}{\theta_{4}(u\tau|\tau)}}.
   \label{theta3}
\end{cases}
\ee
The last terms in the previous equations correspond to the associated Baxter reparametrization of that particular region, expressed in terms of Jacobi theta functions. We have shown this correspondence explicitly for this region in order to persuade the reader that our discrete mappings are nothing but the Baxter reparametrizations. 
In this mapping we have implicitly transformed $u$ (and so $\tilde{z}$) as: $u \rightarrow \frac{u\tau}{\tau+1}$, starting from the left-side of region ${\rm I}_a$. We will show more details about these transformations of $(\tau,u)$ in a specific table later. For the moment we describe how to cover all regions in the upper half-plane by an analytical continuation of formula (\ref{theta2}). Region ${\rm I}_c$ can be reached by doing the same transformation on $(\tau,u)$ as before but starting from the right-side of region ${\rm I}_a$:
\be
\begin{cases}
J_{y}= {\displaystyle\frac{\theta_{3}(\pi (\tau+1)|\tau+1)}{\theta_{2}(\pi (\tau+1)|\tau+1)}}{\displaystyle\frac{\theta_{2}(u\tau|\tau+1)}{\theta_{3}(u\tau|\tau+1)}}\\ 
J_{z}= -{\displaystyle\frac{\theta_{3}(\pi (\tau+1)|\tau+1)}{\theta_{4}(\pi (\tau+1)|\tau+1)}}{\displaystyle\frac{\theta_{4}(u\tau|\tau+1)}{\theta_{3}(u\tau|\tau+1)}}.
   \label{theta4}
\end{cases}
\ee
Then the parametrization of region ${\rm I}_d$ will be splitted up in two subregions, whose parametrization formulae are:
\be
\begin{cases}
J_{y}= {\displaystyle\frac{\theta_{3}(w\left(\frac{\tau}{1+\tau}\right)|\frac{\tau}{1+\tau})}{\theta_{2}(w\left(\frac{\tau}{1+\tau}\right)|\frac{\tau}{1+\tau})}}{\displaystyle\frac{\theta_{2}(\frac{u\tau}{1+\tau}|\frac{\tau}{1+\tau})}{\theta_{3}(\frac{u\tau}{1+\tau}|\frac{\tau}{1+\tau})}}\\
J_{z}= -{\displaystyle\frac{\theta_{3}(w\left(\frac{\tau}{1+\tau}\right)|\frac{\tau}{1+\tau})}{\theta_{4}(w\left(\frac{\tau}{1+\tau}\right)|\frac{\tau}{1+\tau})}}{\displaystyle\frac{\theta_{4}(\frac{u\tau}{1+\tau}|\frac{\tau}{1+\tau})}{\theta_{3}(\frac{u\tau}{1+\tau}|\frac{\tau}{1+\tau})}}.
   \label{theta5}
\end{cases}
\ee
where $w\left(\frac{\tau}{\tau+1}\right) \in \{0,\frac{\pi\tau}{\tau+1}\}$ in the left-side and right-side of region ${\rm I}_d$ respectively.  
In this  mapping we have implicitly transformed $\tau$ as: $\tau \rightarrow \frac{\tau}{\tau+1}$, whilst $u$ remained constant, starting from {\em both} sides of region ${\rm I}_a$.

In figure (\ref{fig:global}) are represented the coordinate curves  of the whole $(J_y,J_z)$ plane.

It is very important to notice that, starting from a point that lies on a particular iso-entropy line in the principal regime, by one of the transformations we listed above 
we reach another point with the {\em same} value of the entropy. This point could belong to the same phase (transformation $\tau \rightarrow \tau + 1$) or to another phase (transformation $\tau \rightarrow \frac{\tau}{\tau+1}$). This is not only true within the first quadrant, as we saw, but it will be true for all transformations we will consider in this section. In the following table we list the coordinates $(\tau,u)$ and $w(\tau)$ we associate to each region, proving that the whole upper half-phase diagram of the XYZ model can be covered with a single parametrization formula, by a suitable choice of the coordinates. Later we will show how these transformations in the parameter space can be generated by two generators only, forming a group. In addition these transformations correspond to Baxter reparametrizations, hence they connect points in the phase diagram with the same Renyi entropy.


\TAVOLA{T1}{List of discrete mappings}{
$$\begin{array}{|c|c|c||c|c|c|}
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm Region} & {\rm Coordinates} &  w(\tau) & {\rm Region} & {\rm Coordinates} & w(\tau)\\ [3mm]
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm I}_a-{\rm (left)} & \left(
\begin{array}{c}
\tau \\
u \\
\end{array}
\right)  & 0 &  {\rm II}_a-{\rm (upper)} & \left(
\begin{array}{c}
-\frac{1}{\tau} \\
u\tau \\ 
\end{array}
\right) & -\frac{\pi}{\tau}  \\ [3mm]
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm I}_a-{\rm (right)} & \left(
\begin{array}{c}
\tau \\
u \\
\end{array}
\right) & \pi\tau &  {\rm IV}_a-{\rm (upper)} & \left(
\begin{array}{c}
-\frac{1}{\tau} \\
u\tau \\
\end{array}
\right) & 0 \\ [3mm]
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm I}_b & \left(
\begin{array}{c}
\tau+1 \\
\frac{u\tau}{\tau+1} \\
\end{array}
\right) & 0 &  {\rm II}_b & \left(
\begin{array}{c}
-\frac{1}{\tau+1} \\
u\tau \\
\end{array}
\right) & -\frac{\pi}{\tau+1} \\ [3mm]
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm I}_c & \left(
\begin{array}{c}
\tau+1 \\
\frac{u\tau}{\tau+1} \\
\end{array}
\right) & \pi(\tau+1) &  {\rm IV}_c & \left(
\begin{array}{c}
-\frac{1}{\tau+1} \\
u\tau \\
\end{array}
\right) & 0 \\ [3mm]
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm I}_d-{\rm (left)} & \left(
\begin{array}{c}
\frac{\tau}{\tau+1} \\
u \\
\end{array}
\right) & 0 &  {\rm II}_d-{\rm (upper)} & \left(
\begin{array}{c}
\frac{\tau-1}{\tau} \\
\frac{u\tau}{\tau-1} \\
\end{array}
\right) & \frac{\pi(\tau-1)}{\tau}  \\ [3mm]
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm I}_d-{\rm (right)} & \left(
\begin{array}{c}
\frac{\tau}{\tau+1} \\
u \\
\end{array}
\right) & \frac{\pi\tau}{\tau+1} &  {\rm IV}_d-{\rm (upper)} & \left(
\begin{array}{c}
\frac{\tau-1}{\tau} \\
\frac{u\tau}{\tau-1} \\
\end{array}
\right) & 0  \\ [3mm]
\hline
\end{array}$$}


\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.45]{long_article8bis.eps}
\par\end{center}
\caption{Coordinate curves of the ($J_y,J_z$) plane.}
\label{fig:global}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Modular transformations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{modulart}

As we noticed in the previous section for the first quadrant, to each discrete mapping it corresponds a modular transformation of the parameter $\tau$. This result still works for all transformations connecting any region of the upper-plane to the principal regime. In this section we will show that, starting from a particular iso-entropy line inside the principal regime, we can generate all other iso-entropy lines in the upper half-phase diagram by applying one of the discrete mappings we listed above. This transformations, that are modular transformations for the parameter $\tau$, can be generated by two different generators acting on the set of parameters $(\tau, u)$. The set of all transformations that may be reduced to successive applications of these generators forms a group, and each element of this group, if seen through its action on the pair $(J_y,J_z)$, acts as a Baxter reparametrization. The novelty of our work lies in the fact that to each Baxter re-arrangement procedure corresponds a {\em discrete} transformation of $(\tau, u)$, and all transformations can be engendered by using two generators only, as we will see below. \\
Here we want to discuss the group properties that are hidden behind the mappings of table (T1). 
% QUESTA NOTA SERVE PER CHIARIRE IL RUOLO DEL DOMINIO FONDAMENTALE NELL'OTTICA DEL GRUPPO G
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Before doing this,
some important remarks are in order. As $(J_y,J_z)$ are always expressed in terms of the Jacobi elliptic funtions cn and dn, and these functions are even in the variable $u$, two different pairs $(\tau, u)$ that differ for the sign of $u$ are to be considered identical. 
 Furthermore if we add $\pm 2\pi$ or $\pm 2\pi\tau$ to $w(\tau)$ we leave  all theta functions unchanged.
 Let us now define the following generators of transformations:
\begin{itemize}
\item Generator T:
\be
\label{T}
T\left(
\begin{array}{c}
\tau \\
u \\
\end{array}
\right)  = \left(
\begin{array}{c}
\tau+1 \\
\frac{u\tau}{\tau+1} \\
\end{array}
\right).
\ee 
\item Generator S:
\be
\label{S}
S\left(
\begin{array}{c}
\tau \\
u \\
\end{array}
\right)  = \left(
\begin{array}{c}
-\frac{1}{\tau} \\
u\tau \\
\end{array}
\right).
\ee 
\end{itemize}

The composition of these generators is defined in the most natural way as the subsequent action of the operators on the resulting triplets. 
For example the action of the operator ST is given by:
\be
\label{example}
ST\left(
\begin{array}{c}
\tau \\
u \\
\end{array}
\right) = \left(
\begin{array}{c}
-\frac{1}{\tau+1}\\
u\tau \\
\end{array}
\right).
\ee 
while the action of TS is given by:
\be
\label{example2}
TS\left(
\begin{array}{c}
\tau \\
u \\
\end{array}
\right) = \left(
\begin{array}{c}
\frac{\tau-1}{\tau}\\
\frac{u\tau}{\tau-1} \\
\end{array}
\right).
\ee 

\begin{figure}[htbp]
\centering%
\subfigure[\protect\url{}\label{fig:modular1}]%
{\includegraphics[scale=0.38]{modular1.eps}}
\subfigure[\protect\url{}\label{fig:modular2}]%
{\includegraphics[scale=0.38]{modular2.eps}}
\caption{Covering of the phase diagram by using the generators $T$, $S$ and $P$.}
\end{figure}

The main algebraic properties of these generators are the following:
\be
\label{algebra}
\begin{cases}
(ST)^{3}=\mathbb{I}\\
S^{2}=\mathbb{I}\\
%P^2=\mathbb{I}\\
%PS=SP\\
%PT=TP
\end{cases}
\ee
where $\mathbb{I}$ is the identity operator. 
Let us now consider the principal regime as a {\em fundamental domain}, where we can move freely in a continuous way. Consider the action of any possible combination of the previous generators on a pair $(\tau, u)$ describing a point inside the principal regime. This set forms a representation of the modular group SL$(2,\mathbb{Z})/\mathbb{Z}_{2}$.
In practice we have found that the set of transformations listed above is homomorphic to the set of Baxter reparametrizations in the upper-half plane. Therefore $S_{\alpha}$ defined in the principal regime as a function of $(\tau, u)$, is invariant under the action of the modular group.\\ 



Let us now consider the problem or parametrizing the lower-half of the phase diagram. The set of transformations needed to implement such a covering is listed in table T2.  

\TAVOLA{T2}{List of discrete mappings}{
$$\begin{array}{|c|c|c||c|c|c|}
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm Region} & {\rm Coordinates} & w(\tau) & {\rm Region} & {\rm Coordinates} & w(\tau)\\ [3mm]
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
%---------------------------------------------------
{\rm III}_a-{\rm (left)} & \left(
\begin{array}{c}
\tau \\
u \\
\end{array}
\right) & \pi & {\rm II}_a-{\rm (lower)} & \left(
\begin{array}{c}
-\frac{1}{\tau} \\
u\tau \\
\end{array}
\right) & \pi -\frac{\pi}{\tau} \\ [3mm] 
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm III}_a-{\rm (right)} & \left(
\begin{array}{c}
\tau \\
u \\
\end{array}
\right) & \pi+\pi\tau &  {\rm IV}_a-{\rm (lower)} & \left(
\begin{array}{c}
-\frac{1}{\tau} \\
u\tau \\
\end{array}
\right) & \pi  \\ [3mm]
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm III}_b & \left(
\begin{array}{c}
\tau+1 \\
\frac{u\tau}{\tau+1} \\
\end{array}
\right) & \pi+\pi(\tau+1) &  {\rm IV}_b & \left(
\begin{array}{c}
-\frac{1}{\tau+1} \\
u\tau \\
\end{array}
\right) & \pi \\ [3mm]
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm III}_c & \left(
\begin{array}{c}
\tau+1 \\
\frac{u\tau}{\tau+1} \\
\end{array}
\right) & \pi &  {\rm II}_c & \left(
\begin{array}{c}
-\frac{1}{\tau+1} \\
u\tau \\
\end{array}
\right) & \pi-\frac{\pi}{\tau+1}  \\ [3mm]
\hline &&&&&\\ [-3mm]
%---------------------------------------------------
{\rm III}_d-{\rm (left)} & \left(
\begin{array}{c}
\frac{\tau}{\tau+1} \\
u \\
\end{array}
\right) & \pi & {\rm II}_d-{\rm (lower)} & \left(
\begin{array}{c}
\frac{\tau-1}{\tau} \\
\frac{u\tau}{\tau-1} \\
\end{array}
\right) & \pi+\frac{\pi(\tau-1)}{\tau}   \\ [3mm]
\hline &&&\\ [-3mm]
%---------------------------------------------------
{\rm III}_d-{\rm (right)} & \left(
\begin{array}{c}
\frac{\tau}{\tau+1} \\
u \\
\end{array}
\right) & \pi+\frac{\pi\tau}{\tau+1} & {\rm IV}_d-{\rm (lower)} & \left(
\begin{array}{c}
\frac{\tau-1}{\tau} \\
\frac{u\tau}{\tau-1} \\
\end{array}
\right) & \pi \\ [3mm]
\hline
\end{array}$$}
%---------------------------------------------------

As we can also see from pictures (\ref{fig:modular1}) and (\ref{fig:modular2}), to cover the region where $J_y \leq 0$ we just need an {\em extra} generator P which acts on the function $w(\tau)$ as $P: (\tau, u; w)\mapsto (\tau, u; w+\pi+\pi\tau)$. In practice to describe the whole phase diagram in its entirety we must consider the action of the generators T,S and P (which also form a group of transformations) on the triplet $(\tau, u; w)$.


%In this formalism $\epsilon$ of formula (\ref{eps2}) is given as a function of the elliptic parameters $(u,\tau)$. Let us suppose that the system is described by the pair $(u',\tau')$ which are connected to their pricipal-regime values by a transformation ${\cal g} \in$ SL$(2,\mathbb{Z})/\mathbb{Z}_{2}$, that is:
%\be
%\label{example}
%{\cal g}\left(
%\begin{array}{c}
%\tau \\
%u \\
%\end{array}
%\right) = \left(
%\begin{array}{c}
%\tau'\\
%u' \\
%\end{array}
%\right).
%\ee 
%	By noticing that the quantity $\eta(\tau)^{24}(u\tau)^{12}$ is invariant under the action of the modular group ($\eta$ is the Dedekind's function), then $\epsilon$ is given by the positive real solution of the following equation:
%\be
%\label{neweps}
%\epsilon^{12}(u',\tau')={\displaystyle\frac{\eta^{24}(\tau')(u'\tau')^{12}}{\eta^{24}(\tau)}}.
%\ee
%Written this way $\epsilon$ can be computed without recalling the parameters $\Gamma$ and $\Delta$ of Baxter parametrization procedure. The only ingredients we need here are the coordinates $(u,\tau)$ of the point plus the transformation that connects that region with the fundamental domain. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analysis of the entropy}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For a quantitative analysis of the Renyi entropy it is now convenient to use the definition of the parameter $\epsilon$ given in (\ref{eps2}), as a function of the parameters $(z,l)$. 
As it is clear from (\ref{eq:renyi4}), the Renyi entropy can be seen as a function of the this parameter only. Then, it is a simple, monotonically decreasing function, such that
\be
   \lim_{\epsilon \to 0} {\cal S}_\alpha = \infty, \qquad \qquad
   \lim_{\epsilon \to \infty} {\cal S}_\alpha = 0.
\ee

However, the behavior of the entropy as a function of the physical parameters of the XYZ model $J_y$ and $J_z$ is more complicated, as they define $z$ and $l$ and thus $\epsilon$. It is worth remarking that the expressions for the entropy given so far apply also for all the other integrable models generated by the R-matrix of the eight-vertex model. For instance, for the XY model one has $\epsilon = \pi  I(l')/I(l)$ and for the XXZ model $\epsilon = \cosh^{-1} J_z$. Compared to these example, the entropy of the XYZ model is more interesting, since it is truly two-dimensional with its independent $l$ and $z$ dependence.

To study the entropy in the $(J_y,J_z)$ phase diagram, we thus need to use (\ref{st11}, \ref{st12}) and to invert (\ref{Iaparameter}) to express   $(z,l)$ as a function of the two parameters $(\Gamma, \Delta)$.
The result was already written in formula (\ref{ste8bis}), that we recall here: 
\begin{equation}
\label{ste8}
    \begin{cases}
     l = \displaystyle{\sqrt{ {1-\Gamma^{2} \over \Delta^{2}-\Gamma^{2} } } }\\
     {\rm dn}(\ii z;l) = \displaystyle{1\over \Gamma}
    \end{cases}
\end{equation}

\begin{figure}[t]
   \begin{center}
      \includegraphics[scale=0.35]{isoentropy1tris.eps}
      \par
   \end{center}
   \caption{Curves of constant entropy of the XYZ model in the ($J_{y},J_{z}$) plane. Regions of similar colors have similar entropy values and the line where colors change are the lines of constant entropy. The brighter is the color, the bigger is the entropy.}
   \label{fig:isoentropy}
\end{figure}

In figure we plot the Von Neumann entropy in the $(J_{y},J_{z})$ plane, for $-2 < J_{y} < 2, -2 < J_{z} < 2$.
This is a contour plot, so regions of similar colors have similar values of the entropy and the line dividing regions of different colors are examples of line of constant entropy.
We immediately see that the entropy draws the same phase diagram we presented in figure \ref{fig:phasediagram}, being singular (diverging) on the critical lines and vanishing on the ferromagnetic Ising lines $(J_y=1,J_z>1)$, $(J_y>1, J_z=1)$, $(|J_y|<1,J_z=J_y)$ and the $J_y \leftrightarrow - J_y$ symmetric ones.

The four tri-critical points $(J_y = \pm 1, J_z = \pm 1)$ are immediately recognized as more interesting and we shall study the entropy in their neighbourhoods in detail.
Let us first look at the conformal point $(J_y = 1, J_z = - 1)$ and use (\ref{ste8}) to write $l$ and $z$.
If we take
\be
   \Gamma = 1 - \rho \cos \phi, \qquad
   \Delta = -1 - \rho \sin \phi, \qquad \qquad
   0 \le \phi \le {\pi \over 2},
\ee
we have
\be
\begin{cases}
   l  =  \left(\tan(\phi)+1\right)^{-1/2}+ {\rm O} \left( \rho \right), \\
   {\rm snh} \left( z ; l\right)  = 
   \sqrt{2\text{cos}(\phi)+2 \text{sin}(\phi)}\,\sqrt{\rho}
   + {\rm O} \left( \rho^{3/2} \right) 
\end{cases}
   \label{vanishinglambda}.
\ee
Thus, $l$ is not defined at the tri-critical point, since its value as $\rho \to 0$ depends on the direction $\phi$ of approach (for $\phi=0$, $l=1$ and for $\phi=\pi/2$, $l=0$).
From (\ref{vanishinglambda}) we see that $z \to 0$ as $\rho \to 0$ and, using $\,\sn (u,l) \simeq u + {\rm O} \left( u^2 \right)$, we find
\be
   z = \sqrt{2\text{cos}(\phi)+2 \text{sin}(\phi)}\,\sqrt{\rho} 
   + {\rm O} \left( \rho^{3/2} \right)
   \label{vanishinglambdabis}.
\ee
Thus, $\epsilon \sim \sqrt{\rho}$ and in any neighbourhood of the conformal point the entropy is diverging.
In particular, on the direction $\phi=0$, since ${\rm I}(1) \to \infty$, the entropy is divergent for any $\rho$ (as expected, since this is a critical line).

Expanding around the other tri-critical point as
\be
   \Gamma = - 1 + \rho \cos \phi, \qquad
   \Delta = -1 - \rho \sin \phi, \qquad \qquad
   0 \le \phi \le {\pi \over 2},
\ee
we find
\be
\begin{cases}
   l  =  \left(\tan(\phi)+1\right)^{-1/2}+ {\rm O} \left( \rho \right), \\
   {\rm snh} \left( z ; l\right)  = 
   -\sqrt{2\text{cos}(\phi)+2 \text{sin}(\phi)}\,\sqrt{\rho}
   + {\rm O} \left( \rho^{3/2} \right)
   
\end{cases}
   \label{singularlambda}\;.
\ee
Thus, $l$ has exactly the same behavior as in the previous case, while ${\rm snh}(z)$ remains unchanged apart from the sign. However in the neighbour of this point we must use the following expansion to extract the limit of $z$, $\,\sn (u,l) \simeq (u-2\ii{\rm I'}) + {\rm O} \left( (u-2\ii{\rm I'})^2 \right)$. This implies $z \sim 2{\rm I'}$ close to $E_{1}$ and thus $\epsilon \sim I(l')/I(l)$, which can take any non-negative value from 0 to $\infty$ for $\phi$ that goes from 0 to $\pi/2$. As we mentioned, the behaviour of the entropy is completely determined by $\epsilon$, thus the Renyi entropy has an essential singularity at $E_{1,2}$, and can take any positive real value in any neighbourhood of it. 

In conclusion, we can say that the points $C_{1,2}$ are  {\em ordinary} critical points, in the sense that in vicinity of this point the Von Neumann block entropy has the universal behavior found in \cite{Cardy}. A detailed study of the entropy near these conformal critical points (and also along the conformal critical lines will be presented in the next chapter).

The behavior of the entropy around the tri-critical points $E_{1,2}$ is clearly quite different. It can be seen directly from the plot that it is direction dependent, since it is an accumulation point for iso-entropy curves. Moreover, it shows a strong discontinuity crossing it along one of the critical lines, since it goes suddenly from diverging to vanishing. In the next sections we will describe the nature of the transition around these points and show that there the entropies have an essential singularity. Another point with the same singular behavior was found at the bi-critical point of the anisotropic XY model in a transverse magnetic field in \cite{Franchini} and was named {\em essential critical point} for the singular behavior of the entropy there.

\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.35]{entropy.eps}
\par\end{center}
\caption{Three-dimensional plot of the Von Neumann block entropy as a function of the coupling constants of the XYZ model. The entanglement entropy diverges when the system is critical.}
\label{fig:entropy}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The essential critical points}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let us now analyze in more details the properties of the ferromagnetic tri-critical points E$_{1,2}$.
Just looking at a blowout of the entropy plot close to this point in figure \ref{fig:isoentropy2} it is evident that depending on the direction of approach the entropy can take any positive value arbitrarily close to it.

\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.25]{isoentropy2.eps}
\par\end{center}
\caption{Curves of constant entropy of the XYZ model in the vicinity of $(J_{y}=1,J_{z}=1)$. We can see that near the essential critical point the lines of constant entropy grow denser. }
\label{fig:isoentropy2}
\end{figure}

This point is very different from all other points along the critical line, because it is not conformal, since low energy excitations are magnons with a quadratic dispersion relation $\varepsilon (q) = 1 - \cos q$. This implies a breakdown of the usual conformal predictions by Calabrese and Cardy \cite{Cardy}.
We showed in the previous sections the singular behavior of the entropy close to this point, since it can take any positive, real value arbitrarily close to it. Moreover, from figure \ref{fig:isoentropy2} one sees that from any point in the phase diagram one can reach one of the non-conformal points following a curve of constant entropy. A point with the same singular behavior for the entropy was already described in \cite{Franchini} as the bi-critical point of the XY model and it was also a non-conformal point with a quadratic dispersion relation.

So far, we studied this point by means of the expressions that we have from the underlying integrable structure. However, it is possible to understand the singular behavior of the entropy in more qualitative, physical terms by looking at the structure of the ground state wavefunction.
At the isotropic point, the Hamiltonian is given by
\begin{equation}
   \hat{H}_{XXX} =
   -{\displaystyle \sum_{n=1}^N} \vec{\sigma}_n \cdot \vec{\sigma}_{n+1} \; .
   \label{eq:XXXH}
\end{equation}
Since $SU(2)$ is unbroken at this point, the Hamiltonian commutes with the generators
\be
   S^2 \equiv {1 \over 4} \sum_{n=1}^N \vec{\sigma}_n \cdot \vec{\sigma}_n \; , \qquad
   S^z \equiv {1 \over 2} \sum_{n=1}^N \vec{\sigma}_n^z \; , \qquad
   S^\pm \equiv {1 \over 2} \sum_{n=1}^N \vec{\sigma}_n^\pm \; .
\ee
Thus, the ground state is $N+1$-fold degenerate, since it is in the representation $S^2 = {N \over 2} \left( {N \over 2} +1 \right)$. This corresponds to a basis of ferromagnetic states, aligned along the different axis. Which state is realized depends on the spontaneous symmetry breaking: a (classical) state aligned in a particular direction will have no entanglement, but a superposition of such states will have an entanglement growing with the number of (classical) states involved.

Hence, we understand that on one of the Ising ferromagnetic lines, the easy-axis anisotropy singles out a classical state as the ground state. Thus, along one of these lines, close to the critical point, the entropy will exactly vanish. In the paramagnetic phases, we have an easy plane anisotropy and thus the ground state is constructed by a large superposition of classical states, yielding a large entropy, diverging in the thermodynamic limit, as prescribed by CFT. In the rest of the phase diagram, we will have an intermediate situation. This qualitative picture helps in interpreting the strong discontinuity in crossing the essential critical point.

Note that the picture is different at the anti-ferromagnetic tri-critical point, since there the ground state always belong to a subspace without finite magnetization and hence it does not go under such a strong discontinuity crossing the tri-critical point. In fact, while a classical ferromagnetic state is an eigenvector of the Hamiltonian anywhere on a ferromagnetic Ising line, a classical Neel state approximates an eigenstate of the AFM Ising line only far from the isotropic point.
From the examples of the XYZ chain and of the XY model \cite{franchini2007}, we can infer that points of discontinuous phase transitions show a characteristic singular behavior of the entanglement entropy, which can be easily detected numerically and might be used as an efficient tool to distinguish, for example, between first and higher order phase transitions in more complicated models \cite{degliesposti2003, franca2008}. It is important to remark that ${\cal S}_\alpha$ and the correlation length show very different behaviors close to $E_{1,2}$, since, as it is expected for any phase transition, $\xi$ diverges as one approaches the critical lines/points, without showing the essential singularity characteristic of the entropy \cite{ercolessi2011}. Thus, close to the discontinuous points $E_{1,2}$ the entropy formula derived in \cite{calabrese2004} is no longer valid: indeed it applies in the vicinity of all conformal points of the critical lines (including the BKT points $C_{1,2}$), while it fails if we are close to non-conformal points, such as $E_{1,2}$ where the spectrum of excitations has a quadratic dispersion relation for small momenta.\\
Let us now try to understand more quantitatively the behaviour of the Renyi entropy in proximity of the essential critical point. Suppose we approach the point E$_{1}$ following a straght line in the $(J_{y},J_{z})$-plane:
\be
\label{eq:essential1}
\begin{cases}
J_{z}=1-t \\
J_{y}=1+m\cdot t,
\end{cases}
\ee
where $t$ is a parameter measuring the distance from E$_{1}$ along a straight line, and $m$ is an angular coefficient such that the path belongs to the principal regime of figure (\ref{fig:phasediagram}). When $t\to 0$ we approach the critical point. Expanding the expressions (\ref{ste8}) for $z$ and $l$ in this limit, we obtain the following expansion for $\epsilon$ (when expanding $z$ and $l$ in the intermediate steps we used the {\em Lagrange inversion theorem} \cite{Lagrange}):
\be  
\label{eq:essential2}
\epsilon=\frac{\pi I\left([(1+m)^{-\frac{1}{2}}]'\right)}{I\left((1+m)^{-\frac{1}{2}}\right)}-\frac{\pi(1+m)^{\frac{1}{2}}}{\sqrt{2}\,I\left((1+m)^{-\frac{1}{2}}\right)}\,t^{\frac{1}{2}}+O(t).
\ee
\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.80]{entropy_essential2.eps}
\par\end{center}
\caption{Behaviour of the Von Neumann entropy along the line (\ref{eq:essential1}) for different values of the angular coefficient $m$.}
\label{fig:entropy_essential}
\end{figure}
Now we want to plug this expression into formula (\ref{eq:modular2}) to obtain the asymptotic behaviour of the Renyi entropy:
\be
\label{eq:essential3}
{\cal S}_{\alpha}={\displaystyle\frac{\alpha\ln(A)-\ln(A_{\alpha})}{6(\alpha-1)}}+\left(\frac{B}{A}+\frac{B_{\alpha}}{A_{\alpha}}\right)\,t^{\frac{1}{2}}+O(t),
\ee
where we clearly see that the entropy saturates to a constant value as we approach the essential critical point. The constants $A$ and $B$ are given by:
\be
\label{eq:essential3}
A={\displaystyle\frac{\theta_{2}(0,{\rm e}^{a})^{2}}{\theta_{3}(0,{\rm e}^{a})\theta_{4}(0,{\rm e}^{a})}},\qquad a=\frac{\pi I\left([(1+m)^{-1/2}]'\right)}{I\left((1+m)^{-1/2}\right)},
\ee
and
\be
\label{eq:essential4}
\begin{array}{lcl}
B & = & -{\displaystyle\left[\theta_{2}(0,{\rm e}^a) \theta_{4}(0,{\rm e}^a) \theta_{3}'(0,{\rm e}^a)+\theta_{2}(0,{\rm e}^a) \theta_{3}(0,{\rm e}^a) \theta_{4}'(0,{\rm e}^a)\right.} \\
& - & {\displaystyle\left. 2\theta_{3}(0,{\rm e}^a) \theta_{4}(0,{\rm e}^a) \theta_{2}'(0,{\rm e}^a)\right]}{\displaystyle\frac{b\,{\rm e}^a \theta_{2}(0,{\rm e}^a)}{\theta_{3}(0,{\rm e}^a)^2 \theta_{4}(0,{\rm e}^a)^2}},
\end{array}
\ee
where $\theta'$ is the derivative of the Jacobi theta function with respect to its second argument and
\be
\label{eq:essential5}
b=-\frac{\pi(1+m)^{1/2}}{\sqrt{2}\,I((1+m)^{-1/2}}.
\ee
$A_{\alpha}$ and $B_{\alpha}$ are obtained from $A$ and $B$ by replacing $a\to\alpha a$ and $b\to\alpha b$. Approaching the essential critical point along a straight line the correlation length diverges as:
\be
\label{eq:essential6}
\xi^{-1}\propto t^{1/2},
\ee
therefore the Renyi entropy goes like:
\be
\label{eq:essential7}
{\cal S}_{\alpha}\approx c_{\alpha}^{1}(m) + c_{\alpha}^{2}(m)\,\xi^{-1/2},
\ee
where $c_{\alpha}^{1}$ and $c_{\alpha}^{2}$ are constants depending on the slope $m$ of the line approaching the critical point. This asymptotic behaviour is very different from the one obtained approaching a conformal critical point and holds true even if we get close to the essential critical point following a parametrization curve with $\tau$ constant.  
\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.80]{invXi.eps}
\par\end{center}
\caption{Behaviour of the inverse of the correlation length $\xi$ along the line (\ref{eq:essential1}) for different values of the angular coefficient $m$.}
\label{fig:invXi_essential}
\end{figure}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Entropy as a function of the Renyi \\ parameter and modular functions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In section (\ref{modulart}) we studied the modular transformations associated to the analytical continuations of the parameters of the model. There we found a family of modular transformations that bridge points with the same value of the Renyi entropy in different phases. 
Now we want to discuss some modular properties of the Renyi entropies, as a function of the parameter $\alpha$ (that was considered constant in the previous sections). 
We will rewrite the Renyi entropy in terms of modular functions, and will note a general property of $S_{\alpha}$ under the action of a particular subgroup of SL$(2,\mathbb{Z})/\mathbb{Z}_{2}$. A similar result was already found for the XY $1/2$ spin chain in a transverse magnetic field, in \cite{Franchini}.
Here we will show that the Renyi entropies of the  XYZ model, from the modular group point of view, have the same properties of those of the  XY $1/2$ spin chain in a transverse magnetic field for $h <2$. 
From expression  (\ref{eq:modular2}) we can rewrite  the Renyi entropy as:
\begin{equation}
S_{\alpha} = 
\frac{\alpha}{6(1-\alpha)} \ln\left(\frac{\theta_{4}(0|\sigma)\theta_{3}(0|\sigma)}{\theta_{2}^{2}(0|\sigma)}  \right)
+\frac{1}{6(1-\alpha)}\ln\left( \frac{\theta_{2}^{2}(0|\alpha \sigma)}{\theta_{3}(0,\alpha \sigma)\theta_{4}(0,\alpha \sigma)}  \right)-\frac{\ln(2)}{3} 
\label{eq:modular9}
\end{equation}
where we use the  parameter $\sigma = {u\tau \over \pi}$.
The functions $\theta_{j}(0|\sigma)$
are holomorphic for  all $\sigma$ of the upper half-plane ${\rm Im}\,\sigma>0$. 
Now it is convenient to introduce the {\em elliptic} $\lambda$ {\em function} or - {\em modular function} as
\begin{equation}
\lambda(\sigma)={\displaystyle\frac{\theta_{2}^{4}(0|\sigma)}{\theta_{3}^{4}(0|\sigma)}}, \quad{\rm Im}\,\sigma >0,
\label{eq:modular13}
\end{equation}
and notice that 
\begin{equation}
1-\lambda(\sigma)={\displaystyle\frac{\theta_{4}^{4}(0|\sigma)}{\theta_{3}^{4}(0|\sigma)}}.
\label{eq:modular14}
\end{equation}
This function play a central role in the theory of modular functions and modular forms (see for instance \cite{Wittaker,Akhiezer,Bateman,Abramowitz}). In term of the modular function, the Renyi entropy can be re-written as
\begin{equation}
S_{\alpha} =\frac{1}{24}\frac{\alpha}{1-\alpha}\ln\left(\frac{\lambda^{2}(\sigma)}{1-\lambda(\sigma)}\right)+ \frac{1}{24}\frac{1}{1-\alpha} \ln\left(\frac{\lambda^{2}(\alpha\sigma)}{1-\lambda(\alpha\sigma)}\right)  -\frac{\ln(2)}{3}.
\label{eq:modular15}
\end{equation}
Now it is natural to introduce the following function:
\begin{equation}
g(\sigma)= {\displaystyle\frac{\lambda^{2}(\sigma)}{1-\lambda(\sigma)}}, 
\label{eq:modular16}
\end{equation}
which allows us to write the Renyi entropy once more in a more compact and clear way:
\begin{equation}
S_{\alpha} =\frac{1}{24}\frac{\alpha}{1-\alpha}\ln[g(\ii \sigma_{0})]+ \frac{1}{24}\frac{1}{1-\alpha} \ln[g(\alpha\ii \sigma_{0})]  -\frac{\ln(2)}{3}
\label{eq:modular17}
\end{equation}
where $\sigma = \ii\sigma_{0}$.
The function $g(\sigma)$ is automorphic with respect to the subgroup of the modular group generated by the two transformations:
\begin{equation}
\sigma \to \sigma +1 \quad {\rm and} \quad \sigma \to \frac{\sigma}{2\sigma+1}.
\label{eq:modular18}
\end{equation}
With these simple observations we arrive at the following general statement:\\ \\ {\em Up to trivial addition terms and multiplicative factors, the Renyi entropy of the XYZ model, as a function of $\alpha$, is an automorphic function with respect to the subgroup  (\ref{eq:modular18}) of the modular group.}\\ \\
In particular, the properties of the modular function $g(\sigma)$ yields, as a special case, the following direct relation between the values of the entropy at points $\alpha$ and $1/\alpha\sigma_{0}^{2}$.
\bea
S_{1/\alpha\sigma_{0}^{2}} & = & {\displaystyle\frac{\alpha\sigma_{0}^{2}}{\alpha\sigma_{0}^{2}-1}}(1-\alpha)S_{\alpha}-\frac{1}{24}{\displaystyle\frac{1-\alpha^{2}\sigma_{0}^{2}}{\alpha\sigma_{0}^{2}-1}}\ln[g(\ii\sigma_{0})] \\
& - & \frac{1}{24} {\displaystyle\frac{\alpha\sigma_{0}^{2}}{\alpha\sigma_{0}^{2}-1}}\ln[f(\alpha\ii\sigma_{0})]+{\displaystyle\frac{1-\alpha^{2}\sigma_{0}^{2}}{\alpha\sigma_{0}^{2}-1}}{\displaystyle\frac{\ln 2}{3}}.
\label{eq:modular20}
\eea
This result concludes the chapter on the general properties of the Renyi entropy of the XYZ model. 


% ------------------------------------------------------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 



==> Chapter3bis/chapter3bis.tex <==
\chapter{The semi-classical method in and out-of-equilibrium}
\ifpdf
    \graphicspath{{Chapter3bis/Chapter3bisFigs/PNG/}{Chapter3bis/Chapter3bisFigs/PDF/}{Chapter3bis/Chapter3bisFigs/}}
\else
    \graphicspath{{Chapter3bis/Chapter3bisFigs/EPS/}{Chapter3bis/Chapter3bisFigs/}}
\fi







\section{The semi-classical theory at finite temperature}
\markboth{\MakeUppercase{\thechapter. The semi-classical method in and out-of-equilibrium}}{\thechapter. The semi-classical method in and out-of-equilibrium}



\subsection{The Potts model}

\subsection{The O(3) non-linear sigma model}

\subsection{The sine-Gordon model}

\section{Semi-classical theory for quantum quenches}

\subsection{The Ising model}

\subsection{The XY model}






% ------------------------------------------------------------------------


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 


==> Conclusions/conclusions.tex <==
\def\baselinestretch{1}
\chapter*{Conclusions}
\ifpdf
    \graphicspath{{Conclusions/ConclusionsFigs/PNG/}{Conclusions/ConclusionsFigs/PDF/}{Conclusions/ConclusionsFigs/}}
\else
    \graphicspath{{Conclusions/ConclusionsFigs/EPS/}{Conclusions/ConclusionsFigs/}}
\fi

\def\baselinestretch{1.66}

Here I put my conclusions ...

%%% ----------------------------------------------------------------------

% ------------------------------------------------------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 


==> Frontpage/frontpage.tex <==
\begin{titlepage}
\begin{center}
\large
UNIVERSIT\`A DI BOLOGNA\\
DIPARTIMENTO DI FISICA ED ASTRONOMIA
\end{center}
\vskip 1.3 truecm
\begin{center}
\Large
Dottorato di Ricerca in Fisica\\
Ciclo XXV
\end{center}
\vskip 1. truecm
\hrule
\begin{center}
\LARGE\bf
QUANTUM CORRELATIONS IN FIELD THEORY
AND INTEGRABLE SYSTEMS\\
\end{center}
\vskip 0.5 truecm
\begin{center}
\Large
Candidato: Stefano Evangelisti
\end{center}
\vskip 0.5 truecm
\begin{center}
%Settore Concorsuale di Appartenenza: 02/A2\\
%Settore Scientifico Disciplinare: FIS/02\\
Settore Concorsuale di Appartenenza: 02/A2\\
Settore Scientifico Disciplinare: FIS/02\\
Coordinatore: Prof. Fabio Ortolani
\end{center}
\hrule
\vskip 1.5 truecm
\begin{center}
\Large
Bologna, 2013
\end{center}
\vskip 1.2 truecm
\begin{center}
\large


\begin{tabular}{l}
Relatore: Prof. Francesco Ravanini \\
Correlatore: Prof. Elisa Ercolessi \\
Correlatore Esterno: Prof. Fabian H.L. Essler (University of Oxford)
%Correlatore esterno: Prof. Fabian H.L. Essler (University of Oxford)
\end{tabular}
\end{center}
\vskip 1.8 truecm



\end{titlepage}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Macros/MacroFile1.tex <==
\newcommand{\PdfPsText}[2]{
  \ifpdf
     #1
  \else
     #2
  \fi
}

\newcommand{\IncludeGraphicsH}[3]{
  \PdfPsText{\includegraphics[height=#2]{#1}}{\includegraphics[bb = #3, height=#2]{#1}}
}

\newcommand{\IncludeGraphicsW}[3]{
  \PdfPsText{\includegraphics[width=#2]{#1}}{\includegraphics[bb = #3, width=#2]{#1}}
}

\newcommand{\InsertFig}[3]{
  \begin{figure}[!htbp]
    \begin{center}
      \leavevmode
      #1
      \caption{#2}
      \label{#3}
    \end{center}
  \end{figure}
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/Documents/LaTeX/CUEDThesisPSnPDF/thesis"
%%% End: 


==> Makefile <==
VERSION=
LATEXTARGET=thesis$(VERSION)

#
# LaTeX Makefile
# --------------
#
# Author : s.m.vandenoord@student.utwente.nl (Stefan van den Oord)
# Date   : March 18, 1999, second version of today.
# 
# This Makefile is a generic makefile for LaTeX documents. Distribute it
# as you wish, but please don't edit or remove this initial comment.
#
# The Makefile can be used by setting the environment variable "MAKEFILES",
# e.g. export MAKEFILES=~/data/TeX/Makefile.
# It requires GNU Make and bash or better, like zsh. Simply sh is not
# sufficient, I believe. The first few lines of the Makefile contains
# the executables that are used, edit them to point to the executables
# on your system.
#
# DISCLAIMER: Using this Makefile is fully at your own risk. I am not
#             responsible for anything! So if crucial files are removed
#             by the Makefile, it is your own problem. But you should
#             have backups anyway. :-)
#
# Usage
# -----
# The Makefile can do the following things for you:
# - generate PostScript equivalents of XFig figures;
# - run makeindex and BibTeX, but only if necessary;
# - compile the .dvi file, running LaTeX as many times as needed;
# - run XDvi with the compiled .dvi file;
# - create a PostScript equivalent of the .dvi file;
# - generate a HTML equivalent of the .dvi file (if Latex2HTML is
#   installed);
# - remove all generated output.
# The Makefile is in some points even RCS aware.
#
# In many cases, you don't even have to tell the Makefile which LaTeX
# file it has to compile. The Makefile uses the following strategy:
# 1. Check if the environment variable LATEXTARGET is set; if it is,
#    generate $LATEXTARGET.dvi.
# 2. If there is only one .tex file, use that one.
# 3. Check if there is a LaTeX file that has the same basename as the
#    directory. For example, if the directory is named "Thesis" and
#    there is a file "Thesis.tex", "Thesis.dvi" is generated.
#
# Invocation
# ----------
# When the MAKEFILES environment variable is set, you can use the
# following commands:
# - make latexhelp
#   Prints an overview of the available commands.
# - make latexfigures
#   Only generate the PostScript equivalents of XFig figures.
# - make file.dvi
#   Generates the specified DVI file.
# - make file.ps
#   Generates the DVI file and then runs dvips.
# - make latex
#   Use the above explained strategy to find out what has to be
#   generated, and generate it.
# - make view
#   Do a make latex and then run XDvi.
# - make latexps
#   Do a make latex and then run dvips.
# - make html
#   Do a make latex and then use LaTeX2HTML to create the HTML equivalent.
#   To do this, the following environment variables are used:
#   * HTMLDIR : the base dir in which the output is written. For example,
#               if HTMLDIR=~/public_html/LaTeX, and the file that is
#               generated is "Thesis", the output will be written in the
#               directory ~/public_html/LaTeX/Thesis.
#   * LATEX2HTML_OPTS : if you want to pass options to LaTeX2HTML, put
#                       them in this variable.
# - make latexclean
#   This command removes all generated output. CAUTION: the files that are
#   removed are thought out pretty well, but it is possible that files are
#   removed that you wanted to keep! Check below what files are removed if
#   you want to be certain!
#   Note that a file figure.eps is only removed if a file figure.fig exists.
#   (Even if the file figure.fig exists, but is checked in using RCS, the
#   file figure.eps will be removed.)
#
# Tip
# ---
# For some projects it is useful to have a separate Makefile in the project's
# directory. For example, when you use RCS, you could add functionality for
# automatic checkouts of the right files (adding dependencies is sufficient;
# GNU Make rocks :-).
# The command "latexclean" is declared so that you can add your own
# functionality in the project's Makefile; instead of one colon, declare it
# with two colons if you want to do that.
# For example:
# latexclean::
#     rm -f foo.bar
# This way both the origional definition in this Makefile and your own are
# used.

#.SILENT:

# SHELL=/usr/local/bin/bash

LATEX=latex
PDFLATEX=pdflatex
BIBTEX=bibtex
DVIPS=dvips
MAKEINDEX=makeindex
DVIVIEWER=xdvi -geometry 710x950-0+10
LATEX2HTML=latex2html

FIGURES=$(wildcard *.fig)
FIGUREOBJS=$(FIGURES:.fig=.eps)

TEXFILES=$(wildcard *.tex)

# Disable standard pattern rule:
%.dvi: %.tex

# Do not delete the following targets:
.PRECIOUS: %.aux %.bbl %.eps %.ind

%.aux: %.tex $(FIGUREOBJS) $(TEXFILES)
	@$(LATEX) $*
# Look for citations. Make sure grep never returns an error code.
	@grep "^\\\\citation" *.aux > .btmp.new || true

# If the citations are not changed, don't do anything. Otherwise replace
# the .btmp file to make sure Bibtex will be run.
	@if ( diff .btmp.new .btmp >& /dev/null ); then \
		rm .btmp.new; \
	else \
		mv .btmp.new .btmp; \
	fi

	@if [ -f $*.idx ]; then cp $*.idx .itmp.new; else touch .itmp.new; fi
	@if ( diff .itmp.new .itmp >& /dev/null ); then \
		rm .itmp.new; \
	else \
		mv .itmp.new .itmp; \
	fi

.btmp:

%.bbl: $(BIBFILES) .btmp
# Only use BibTeX if \bibliography occurs in the document. In that case,
# run BibTeX and recompile. .btmp is touched to prevent useless making
# next time.
	@if ( grep "^\\\\bibliography{" $*.tex > /dev/null ); then \
		$(BIBTEX) $*; \
		touch .rerun; \
	fi
	@touch .btmp

.itmp:

%.ind: .itmp
	@if [ -f $*.idx ]; then \
		$(MAKEINDEX) $*; \
		touch .rerun; \
		touch .itmp; \
	fi

%.eps:%.fig
	@echo Generating figure $@...
	@fig2dev -L ps $< $@

%.dvi: %.aux %.ind %.bbl
# Make sure the dvi-file exists; if not: recompile.
	@if [ ! -f $*.dvi ]; then \
		touch .rerun; \
	fi

	@if [ -f .rerun ]; then \
		rm .rerun; \
		$(LATEX) $*; \
	else \
		$(MAKE) $*.aux; \
	fi

# While references et al. are changed: recompile.
	@while ( grep Rerun $*.log > /dev/null ); do \
		$(LATEX) $*; \
	done

# Touch the figureobjects to prevent making next time
	@if [ -n "$(FIGUREOBJS)" ]; then \
		touch $(FIGUREOBJS); \
		touch $*.aux; \
	fi

	@if [ -f $*.ind ]; then \
		touch $*.ind; \
	fi
	@$(MAKEINDEX) -s nomencl.ist -o $*.nls $*.nlo

latex:
# Below the 'true' is included to prevent unnecessarily many errors.
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.dvi; \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.dvi; \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.dvi; \
			true; \
		fi; \
	fi

latexfigures:
	@for i in $(FIGUREOBJS); do \
		$(MAKE) $$i; \
	done

view:
# Below the 'true' is included to prevent unnecessarily many errors.
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.dvi && \
		$(DVIVIEWER) ${LATEXTARGET}.dvi ; \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.dvi && \
			$(DVIVIEWER) `basename \`ls *.tex\` .tex`.dvi; \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.dvi && \
			$(DVIVIEWER) `echo $$PWD|tr '/' '\n'|tail -1`.dvi; \
			true; \
		fi; \
	fi

%.ps: %.dvi
	$(DVIPS) -o $*.ps $<
	@$(MAKEINDEX) -s nomencl.ist -o $*.nls $*.nlo
	$(DVIPS) -o $*.ps $<

%.pdf: %.tex
	$(PDFLATEX) $<
	@$(MAKEINDEX) -s nomencl.ist -o $*.nls $*.nlo
	$(BIBTEX) $*
	$(PDFLATEX) $<
	$(PDFLATEX) $<

latexps:
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.ps && \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.ps && \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.ps && \
			true; \
		fi; \
	fi

html: .html

.html:
	@if [ -n "${LATEXTARGET}" ]; then \
		if [ -n "${HTMLDIR}" ]; then \
			$(MAKE) ${LATEXTARGET}.dvi; \
			$(LATEX2HTML) $(LATEX2HTML_OPTS) -dir $(HTMLDIR)/$(LATEXTARGET) $(LATEXTARGET) && \
			chmod a+rx $(HTMLDIR)/$(LATEXTARGET) && \
			chmod a+r $(HTMLDIR)/$(LATEXTARGET)/* &&  \
			touch .html; \
		else \
			echo Set variable HTMLDIR\!; \
		fi; \
	else \
		echo Set variable LATEXTARGET\!; \
	fi

latexhelp:
	@echo "LaTeX Makefile Options"
	@echo "----------------------"
	@echo ""
	@echo "Environment variables:"
	@echo "  LATEXTARGET   Filename to make (without extension)"
	@echo "  HTMLDIR       Directory for HTML-output"
	@echo "  FIGURES       Figures that have to be compiled"
	@echo ""
	@echo "Targets:"
	@echo "  all           Make the LATEXTARGET or <dirname>.dvi"
	@echo "  <name>.dvi    Make the given dvi file"
	@echo "  latex         Make the LATEXTARGET or <dirname>.dvi"
	@echo "  view          Make and view the LATEXTARGET or <dirname>.dvi"
	@echo "  html          Make the LATEXTARGET  or <dirname>.dvi and generate HTML output"
	@echo "  latexhelp     This overview"
	@echo "  latexclean    Remove all generated files"

clean latexclean::
	@rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.out *.brf *.html *.btmp *.itmp *.rerun *.glo *.gls *.nlo *.nls
	@epsfiles=`find * -maxdepth 0  -name "*.eps" `; \
	if [ -n "$$epsfiles" ]; then \
		for i in *.eps; do \
			if [ -f `basename $$i .eps`.fig ]; then \
				rm -f $$i; \
			elif ( rcs `basename $$i .eps`.fig >& /dev/null ); then \
				rm -f $$i; \
			fi \
		done \
	fi

cleanpspdf : clean
	@rm -f *.ps *.pdf

clobber : cleanpspdf
	@rm -f *~

